Fixed-Target Runtime Analysis

Runtime analysis aims at contributing to our understanding of evolutionary algorithms through mathematical analyses of their runtimes. In the context of discrete optimization problems, runtime analysis classically studies the time needed to find an optimal solution. However, both from a practical and from a theoretical viewpoint, more fine-grained performance measures are needed to gain a more detailed understanding of the main working principles and their resulting performance implications. Two complementary approaches have been suggested: fixed-budget analyses and fixed-target analyses. In this work, we conduct an in-depth study on the advantages and the limitations of fixed-target analyses. We show that, different from fixed-budget analyses, many classical methods from the runtime analysis of discrete evolutionary algorithms yield fixed-target results without greater effort. We use this to conduct a number of new fixed-target analyses. However, we also point out examples where an extension of existing runtime results to fixed-target results is highly non-trivial.

==> figures/figure-om-new.tex <==
\begin{tikzpicture}
\begin{axis}[width=\onemaxplotwidthleftnew, height=\onemaxplotheight, enlargelimits=false, grid=major, ymode=log, xlabel={Relative fitness, $n = 10^3$}, ylabel={Evaluations},
             cycle list name=onemaxplotcyclenew, legend pos=outer north east]
    \addplot+ coordinates {(0.00,1.000000)(0.01,1.000000)(0.02,1.000000)(0.03,1.000000)(0.04,1.000000)(0.05,1.000000)(0.06,1.000000)(0.07,1.000000)(0.08,1.000000)(0.09,1.000000)(0.10,1.000000)(0.11,1.000000)(0.12,1.000000)(0.13,1.000000)(0.14,1.000000)(0.15,1.000000)(0.16,1.000000)(0.17,1.000000)(0.18,1.000000)(0.19,1.000000)(0.20,1.000000)(0.21,1.000000)(0.22,1.000000)(0.23,1.000000)(0.24,1.000000)(0.25,1.000000)(0.26,1.000000)(0.27,1.000000)(0.28,1.000000)(0.29,1.000000)(0.30,1.000000)(0.31,1.000000)(0.32,1.000000)(0.33,1.000000)(0.34,1.000000)(0.35,1.000000)(0.36,1.000000)(0.37,1.000000)(0.38,1.000000)(0.39,1.000000)(0.40,1.000000)(0.41,1.000000)(0.42,1.000001)(0.43,1.000039)(0.44,1.000709)(0.45,1.008924)(0.46,1.078423)(0.47,1.488187)(0.48,3.193164)(0.49,8.288503)(0.50,19.509220)(0.51,38.415837)(0.52,64.118490)(0.53,94.239361)(0.54,126.761255)(0.55,160.728946)(0.56,195.886664)(0.57,232.229916)(0.58,269.812687)(0.59,308.701311)(0.60,348.967982)(0.61,390.690616)(0.62,433.953399)(0.63,478.847464)(0.64,525.471657)(0.65,573.933413)(0.66,624.349757)(0.67,676.848457)(0.68,731.569355)(0.69,788.665907)(0.70,848.306976)(0.71,910.678930)(0.72,975.988110)(0.73,1044.463742)(0.74,1116.361400)(0.75,1191.967152)(0.76,1271.602545)(0.77,1355.630652)(0.78,1444.463467)(0.79,1538.571013)(0.80,1638.492666)(0.81,1744.851390)(0.82,1858.371806)(0.83,1979.903418)(0.84,2110.450877)(0.85,2251.213982)(0.86,2403.641468)(0.87,2569.504683)(0.88,2751.000704)(0.89,2950.900222)(0.90,3172.765793)(0.91,3421.284841)(0.92,3702.798473)(0.93,4026.182850)(0.94,4404.409237)(0.95,4857.525924)(0.96,5418.971350)(0.97,6151.006170)(0.98,7191.773108)(0.99,8970.510079)(1.00,16895.689296)};
    \addlegendentry{\small $(1+1)$ EA rand};
    \addplot+ coordinates {(0.00,1.00)(0.01,1.00)(0.02,1.00)(0.03,1.00)(0.04,1.00)(0.05,1.00)(0.06,1.00)(0.07,1.00)(0.08,1.00)(0.09,1.00)(0.10,1.00)(0.11,1.00)(0.12,1.00)(0.13,1.00)(0.14,1.00)(0.15,1.00)(0.16,1.00)(0.17,1.00)(0.18,1.00)(0.19,1.00)(0.20,1.00)(0.21,1.00)(0.22,1.00)(0.23,1.00)(0.24,1.00)(0.25,1.00)(0.26,1.00)(0.27,1.00)(0.28,1.00)(0.29,1.00)(0.30,1.00)(0.31,1.00)(0.32,1.00)(0.33,1.00)(0.34,1.00)(0.35,1.00)(0.36,1.00)(0.37,1.00)(0.38,1.00)(0.39,1.00)(0.40,1.00)(0.41,1.00)(0.42,1.00)(0.43,1.00)(0.44,1.00)(0.45,1.00)(0.46,1.00)(0.47,1.00)(0.48,1.00)(0.49,1.00)(0.50,1.00)(0.51,1.00)(0.52,1.00)(0.53,1.00)(0.54,1.00)(0.55,1.00)(0.56,1.00)(0.57,1.00)(0.58,1.00)(0.59,1.00)(0.60,1.00)(0.61,1.00)(0.62,1.00)(0.63,1.00)(0.64,1.00)(0.65,1.00)(0.66,1.00)(0.67,2.42)(0.68,9.97)(0.69,18.00)(0.70,26.55)(0.71,35.68)(0.72,45.44)(0.73,55.89)(0.74,67.12)(0.75,79.19)(0.76,92.22)(0.77,106.31)(0.78,121.59)(0.79,138.22)(0.80,156.37)(0.81,176.26)(0.82,198.15)(0.83,222.33)(0.84,249.18)(0.85,279.15)(0.86,312.82)(0.87,350.90)(0.88,394.30)(0.89,444.21)(0.90,502.20)(0.91,570.40)(0.92,651.78)(0.93,750.63)(0.94,873.38)(0.95,1030.22)(0.96,1238.50)(0.97,1530.99)(0.98,1980.35)(0.99,2806.03)(1.00,7330.34)};
    \addlegendentry{\small Our result};
    \addplot+ coordinates {(0.0,1.0)(0.01,1.0)(0.02,1.0)(0.03,1.0)(0.04,1.0)(0.05,1.0)(0.06,1.0)(0.07,1.0)(0.08,1.0)(0.09,1.0)(0.1,1.0)(0.11,1.0)(0.12,1.0)(0.13,1.0)(0.14,1.0)(0.15,1.0)(0.16,1.0)(0.17,1.0)(0.18,1.0)(0.19,1.0)(0.2,1.0)(0.21,1.0)(0.22,1.0)(0.23,1.0)(0.24,1.0)(0.25,1.0)(0.26,1.0)(0.27,1.0)(0.28,1.0)(0.29,1.0)(0.3,1.0)(0.31,1.0)(0.32,1.0)(0.33,1.0)(0.34,1.0)(0.35,1.0)(0.36,1.0)(0.37,1.0)(0.38,1.0)(0.39,1.0)(0.4,1.0)(0.41,1.0)(0.42,1.0)(0.43,1.0)(0.44,1.0)(0.45,1.0)(0.46,1.0)(0.47,1.0)(0.48,1.0)(0.49,1.0)(0.5,1.0)(0.51,1.0)(0.52,1.0)(0.53,1.0)(0.54,1.0)(0.55,1.0)(0.56,1.0)(0.57,1.0)(0.58,1.0)(0.59,1.0)(0.6,1.0)(0.61,1.0)(0.62,1.0)(0.63,1.0)(0.64,1.0)(0.65,1.0)(0.66,1.0)(0.67,1.0)(0.68,1.0)(0.69,1.0)(0.7,1.0)(0.71,1.0)(0.72,1.0)(0.73,1.0)(0.74,1.0)(0.75,1.0)(0.76,1.0)(0.77,1.0)(0.78,1.0)(0.79,1.0)(0.8,1.0)(0.81,1.0)(0.82,1.0)(0.83,1.0)(0.84,1.0)(0.85,1.0)(0.86,1.0)(0.87,1.0)(0.88,1.0)(0.89,1.0)(0.9,1.0)(0.91,1.0)(0.92,1.0)(0.93,1.0)(0.94,1.0)(0.95,1.0)(0.96,1.0)(0.97,1.0)(0.98,1.0)(0.99,1.0)(1.0,1.0)};
    \addlegendentry{\small Lower bound, LS};
\end{axis}
\end{tikzpicture}
\par
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}
\begin{axis}[width=\onemaxplotwidthleftnew, height=\onemaxplotheight, enlargelimits=false, grid=major, ymode=log, xlabel={Relative fitness, $n = 10^4$}, ylabel={Evaluations},
             cycle list name=onemaxplotcyclenew]
    \addplot+ coordinates {(0.00,1.000000)(0.01,1.000000)(0.02,1.000000)(0.03,1.000000)(0.04,1.000000)(0.05,1.000000)(0.06,1.000000)(0.07,1.000000)(0.08,1.000000)(0.09,1.000000)(0.10,1.000000)(0.11,1.000000)(0.12,1.000000)(0.13,1.000000)(0.14,1.000000)(0.15,1.000000)(0.16,1.000000)(0.17,1.000000)(0.18,1.000000)(0.19,1.000000)(0.20,1.000000)(0.21,1.000000)(0.22,1.000000)(0.23,1.000000)(0.24,1.000000)(0.25,1.000000)(0.26,1.000000)(0.27,1.000000)(0.28,1.000000)(0.29,1.000000)(0.30,1.000000)(0.31,1.000000)(0.32,1.000000)(0.33,1.000000)(0.34,1.000000)(0.35,1.000000)(0.36,1.000000)(0.37,1.000000)(0.38,1.000000)(0.39,1.000000)(0.40,1.000000)(0.41,1.000000)(0.42,1.000000)(0.43,1.000000)(0.44,1.000000)(0.45,1.000000)(0.46,1.000000)(0.47,1.000000)(0.48,1.001016)(0.49,2.232958)(0.50,60.019541)(0.51,303.211508)(0.52,612.462965)(0.53,932.677202)(0.54,1263.045214)(0.55,1604.074142)(0.56,1956.307983)(0.57,2320.329829)(0.58,2696.765584)(0.59,3086.288154)(0.60,3489.622133)(0.61,3907.549105)(0.62,4340.913618)(0.63,4790.629976)(0.64,5257.689945)(0.65,5743.171562)(0.66,6248.249220)(0.67,6774.205256)(0.68,7322.443332)(0.69,7894.503941)(0.70,8492.082464)(0.71,9117.050287)(0.72,9771.479633)(0.73,10457.672911)(0.74,11178.197619)(0.75,11935.928091)(0.76,12734.095783)(0.77,13576.350261)(0.78,14466.833771)(0.79,15410.273166)(0.80,16412.094277)(0.81,17478.565659)(0.82,18616.981228)(0.83,19835.895157)(0.84,21145.428059)(0.85,22557.672104)(0.86,24087.236077)(0.87,25751.992746)(0.88,27574.125864)(0.89,29581.633676)(0.90,31810.550726)(0.91,34308.343696)(0.92,37139.314634)(0.93,40393.628755)(0.94,44203.343203)(0.95,48773.168675)(0.96,54445.955033)(0.97,61864.061373)(0.98,72468.018320)(0.99,90842.430138)(1.00,231451.709430)};
    \addplot+ coordinates {(0.00,1.00)(0.01,1.00)(0.02,1.00)(0.03,1.00)(0.04,1.00)(0.05,1.00)(0.06,1.00)(0.07,1.00)(0.08,1.00)(0.09,1.00)(0.10,1.00)(0.11,1.00)(0.12,1.00)(0.13,1.00)(0.14,1.00)(0.15,1.00)(0.16,1.00)(0.17,1.00)(0.18,1.00)(0.19,1.00)(0.20,1.00)(0.21,1.00)(0.22,1.00)(0.23,1.00)(0.24,1.00)(0.25,1.00)(0.26,1.00)(0.27,1.00)(0.28,1.00)(0.29,1.00)(0.30,1.00)(0.31,1.00)(0.32,1.00)(0.33,1.00)(0.34,1.00)(0.35,1.00)(0.36,1.00)(0.37,1.00)(0.38,1.00)(0.39,1.00)(0.40,1.00)(0.41,1.00)(0.42,1.00)(0.43,1.00)(0.44,1.00)(0.45,1.00)(0.46,1.00)(0.47,1.00)(0.48,1.00)(0.49,1.00)(0.50,1.00)(0.51,1.00)(0.52,1.00)(0.53,1.00)(0.54,1.00)(0.55,1.00)(0.56,1.00)(0.57,1.00)(0.58,1.00)(0.59,1.00)(0.60,1.00)(0.61,1.00)(0.62,1.00)(0.63,1.00)(0.64,1.00)(0.65,1.00)(0.66,1.00)(0.67,36.80)(0.68,151.47)(0.69,273.01)(0.70,402.05)(0.71,539.28)(0.72,685.52)(0.73,841.68)(0.74,1008.79)(0.75,1188.04)(0.76,1380.79)(0.77,1588.63)(0.78,1813.38)(0.79,2057.20)(0.80,2322.61)(0.81,2612.59)(0.82,2930.75)(0.83,3281.37)(0.84,3669.72)(0.85,4102.25)(0.86,4586.97)(0.87,5134.01)(0.88,5756.33)(0.89,6470.77)(0.90,7299.74)(0.91,8273.71)(0.92,9435.28)(0.93,10846.14)(0.94,12599.49)(0.95,14844.13)(0.96,17836.01)(0.97,22065.10)(0.98,28643.39)(0.99,41075.30)(1.00,133711.25)};
    \addplot+ coordinates {(0.0,1.0)(0.01,1.0)(0.02,1.0)(0.03,1.0)(0.04,1.0)(0.05,1.0)(0.06,1.0)(0.07,1.0)(0.08,1.0)(0.09,1.0)(0.1,1.0)(0.11,1.0)(0.12,1.0)(0.13,1.0)(0.14,1.0)(0.15,1.0)(0.16,1.0)(0.17,1.0)(0.18,1.0)(0.19,1.0)(0.2,1.0)(0.21,1.0)(0.22,1.0)(0.23,1.0)(0.24,1.0)(0.25,1.0)(0.26,1.0)(0.27,1.0)(0.28,1.0)(0.29,1.0)(0.3,1.0)(0.31,1.0)(0.32,1.0)(0.33,1.0)(0.34,1.0)(0.35,1.0)(0.36,1.0)(0.37,1.0)(0.38,1.0)(0.39,1.0)(0.4,1.0)(0.41,1.0)(0.42,1.0)(0.43,1.0)(0.44,1.0)(0.45,1.0)(0.46,1.0)(0.47,1.0)(0.48,1.0)(0.49,1.0)(0.5,1.0)(0.51,1.0)(0.52,1.0)(0.53,1.0)(0.54,1.0)(0.55,1.0)(0.56,1.0)(0.57,1.0)(0.58,1.0)(0.59,1.0)(0.6,1.0)(0.61,1.0)(0.62,1.0)(0.63,1.0)(0.64,1.0)(0.65,1.0)(0.66,1.0)(0.67,1.0)(0.68,1.0)(0.69,1.0)(0.7,1.0)(0.71,1.0)(0.72,1.0)(0.73,1.0)(0.74,1.0)(0.75,1.0)(0.76,1.0)(0.77,1.0)(0.78,1.0)(0.79,1.0)(0.8,1.0)(0.81,1.0)(0.82,1.0)(0.83,1.0)(0.84,1.0)(0.85,1.0)(0.86,1.0)(0.87,1.0)(0.88,1.0)(0.89,1.0)(0.9,1.0)(0.91,1.0)(0.92,1.0)(0.93,1.0)(0.94,1.0)(0.95,1.0)(0.96,1.0)(0.97,1.0)(0.98,1.0)(0.99,1.0)(1.0,45956.47254329891)};
\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis}[width=\onemaxplotwidthright, height=\onemaxplotheight, enlargelimits=false, grid=major, ymode=log, xlabel={\phantom{Rf, $n = 10^4$}},
             cycle list name=onemaxplotcyclenew,
             x tick label style={/pgf/number format/fixed,/pgf/number format/precision=3}]
    \addplot+ coordinates {(0.9975,127819.815525)(0.9976,128903.116938)(0.9977,130031.724818)(0.9978,131209.578901)(0.9979,132441.156159)(0.9980,133731.573133)(0.9981,135086.713842)(0.9982,136513.391366)(0.9983,138019.554292)(0.9984,139614.553904)(0.9985,141309.494849)(0.9986,143117.702705)(0.9987,145055.358529)(0.9988,147142.377470)(0.9989,149403.653463)(0.9990,151870.869700)(0.9991,154585.214327)(0.9992,157601.604876)(0.9993,160995.552952)(0.9994,164874.932275)(0.9995,169401.553428)(0.9996,174834.313340)(0.9997,181626.281641)(0.9998,190683.597588)(0.9999,204271.609325)(1.0000,231451.709430)};
    \addplot+ coordinates {(0.9975,67085.14)(0.9976,67825.88)(0.9977,68595.03)(0.9978,69394.85)(0.9979,70227.90)(0.9980,71097.06)(0.9981,72005.63)(0.9982,72957.41)(0.9983,73956.76)(0.9984,75008.77)(0.9985,76119.45)(0.9986,77295.88)(0.9987,78546.59)(0.9988,79881.95)(0.9989,81314.73)(0.9990,82860.97)(0.9991,84541.21)(0.9992,86382.39)(0.9993,88420.97)(0.9994,90708.13)(0.9995,93319.35)(0.9996,96373.60)(0.9997,100077.08)(0.9998,104845.70)(0.9999,111798.05)(1.0000,133711.25)};
    \addplot+ coordinates {(0.9975,1.0)(0.9976,1.0)(0.9977,1.0)(0.9978,1.0)(0.9979,1.0)(0.998,1.0)(0.9981,1.0)(0.9982,1.0)(0.9983,1.0)(0.9984,1.0)(0.9985,1.0)(0.9986,1.0)(0.9987,1.0)(0.9988,1.0)(0.9989,1.0)(0.999,1.0)(0.9991,1.0)(0.9992,1.0)(0.9993,1.0)(0.9994,1.0)(0.9995,1.0)(0.9996,2207.414229272137)(0.9997,8273.08483602447)(0.9998,16093.094335215603)(0.9999,27114.778689661704)(1.0,45956.47254329891)};
\end{axis}
\end{tikzpicture}
\par
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}
\begin{axis}[width=\onemaxplotwidthleftnew, height=\onemaxplotheight, enlargelimits=false, grid=major, ymode=log, xlabel={Relative fitness, $n = 10^5$}, ylabel={Evaluations},
             cycle list name=onemaxplotcyclenew]
    \addplot+ coordinates {(0.00,1.000000)(0.01,1.000000)(0.02,1.000000)(0.03,1.000000)(0.04,1.000000)(0.05,1.000000)(0.06,1.000000)(0.07,1.000000)(0.08,1.000000)(0.09,1.000000)(0.10,1.000000)(0.11,1.000000)(0.12,1.000000)(0.13,1.000000)(0.14,1.000000)(0.15,1.000000)(0.16,1.000000)(0.17,1.000000)(0.18,1.000000)(0.19,1.000000)(0.20,1.000000)(0.21,1.000000)(0.22,1.000000)(0.23,1.000000)(0.24,1.000000)(0.25,1.000000)(0.26,1.000000)(0.27,1.000000)(0.28,1.000000)(0.29,1.000000)(0.30,1.000000)(0.31,1.000000)(0.32,1.000000)(0.33,1.000000)(0.34,1.000000)(0.35,1.000000)(0.36,1.000000)(0.37,1.000000)(0.38,1.000000)(0.39,1.000000)(0.40,1.000000)(0.41,1.000000)(0.42,1.000000)(0.43,1.000000)(0.44,1.000000)(0.45,1.000000)(0.46,1.000000)(0.47,1.000000)(0.48,1.000000)(0.49,1.000000)(0.50,188.073696)(0.51,3014.133821)(0.52,6119.986451)(0.53,9322.630291)(0.54,12626.821342)(0.55,16037.643404)(0.56,19560.537968)(0.57,23201.337575)(0.58,26966.303101)(0.59,30862.165570)(0.60,34896.173131)(0.61,39076.144025)(0.62,43410.526433)(0.63,47908.466348)(0.64,52579.884757)(0.65,57435.565741)(0.66,62487.257361)(0.67,67747.787650)(0.68,73231.198482)(0.69,78952.900750)(0.70,84929.855017)(0.71,91180.782853)(0.72,97726.415320)(0.73,104589.786699)(0.74,111796.583740)(0.75,119375.563486)(0.76,127359.056507)(0.77,135783.577350)(0.78,144690.570842)(0.79,154127.332209)(0.80,164148.151930)(0.81,174815.754590)(0.82,186203.127217)(0.83,198395.870861)(0.84,211495.266050)(0.85,225622.328996)(0.86,240923.269515)(0.87,257576.975244)(0.88,275805.497754)(0.89,295889.112302)(0.90,318188.575627)(0.91,343179.150660)(0.92,371504.754998)(0.93,404068.455264)(0.94,442193.188198)(0.95,487930.332357)(0.96,544716.957384)(0.97,618996.716937)(0.98,725235.286787)(0.99,909581.286452)(1.00,2940300.675484)};
    \addplot+ coordinates {(0.00,1.00)(0.01,1.00)(0.02,1.00)(0.03,1.00)(0.04,1.00)(0.05,1.00)(0.06,1.00)(0.07,1.00)(0.08,1.00)(0.09,1.00)(0.10,1.00)(0.11,1.00)(0.12,1.00)(0.13,1.00)(0.14,1.00)(0.15,1.00)(0.16,1.00)(0.17,1.00)(0.18,1.00)(0.19,1.00)(0.20,1.00)(0.21,1.00)(0.22,1.00)(0.23,1.00)(0.24,1.00)(0.25,1.00)(0.26,1.00)(0.27,1.00)(0.28,1.00)(0.29,1.00)(0.30,1.00)(0.31,1.00)(0.32,1.00)(0.33,1.00)(0.34,1.00)(0.35,1.00)(0.36,1.00)(0.37,1.00)(0.38,1.00)(0.39,1.00)(0.40,1.00)(0.41,1.00)(0.42,1.00)(0.43,1.00)(0.44,1.00)(0.45,1.00)(0.46,1.00)(0.47,1.00)(0.48,1.00)(0.49,1.00)(0.50,1.00)(0.51,1.00)(0.52,1.00)(0.53,1.00)(0.54,1.00)(0.55,1.00)(0.56,1.00)(0.57,1.00)(0.58,1.00)(0.59,1.00)(0.60,1.00)(0.61,1.00)(0.62,1.00)(0.63,1.00)(0.64,1.00)(0.65,1.00)(0.66,1.00)(0.67,412.06)(0.68,1695.68)(0.69,3055.42)(0.70,4498.23)(0.71,6031.99)(0.72,7665.55)(0.73,9409.01)(0.74,11273.85)(0.75,13273.21)(0.76,15422.23)(0.77,17738.39)(0.78,20242.03)(0.79,22956.95)(0.80,25911.18)(0.81,29137.95)(0.82,32677.00)(0.83,36576.25)(0.84,40894.03)(0.85,45702.12)(0.86,51089.88)(0.87,57170.06)(0.88,64087.11)(0.89,72029.36)(0.90,81247.31)(0.91,92082.21)(0.92,105012.36)(0.93,120731.81)(0.94,140292.23)(0.95,165379.27)(0.96,198907.36)(0.97,246497.44)(0.98,321057.84)(0.99,464226.00)(1.00,1955749.24)};
    \addplot+ coordinates {(0.0,1.0)(0.01,1.0)(0.02,1.0)(0.03,1.0)(0.04,1.0)(0.05,1.0)(0.06,1.0)(0.07,1.0)(0.08,1.0)(0.09,1.0)(0.1,1.0)(0.11,1.0)(0.12,1.0)(0.13,1.0)(0.14,1.0)(0.15,1.0)(0.16,1.0)(0.17,1.0)(0.18,1.0)(0.19,1.0)(0.2,1.0)(0.21,1.0)(0.22,1.0)(0.23,1.0)(0.24,1.0)(0.25,1.0)(0.26,1.0)(0.27,1.0)(0.28,1.0)(0.29,1.0)(0.3,1.0)(0.31,1.0)(0.32,1.0)(0.33,1.0)(0.34,1.0)(0.35,1.0)(0.36,1.0)(0.37,1.0)(0.38,1.0)(0.39,1.0)(0.4,1.0)(0.41,1.0)(0.42,1.0)(0.43,1.0)(0.44,1.0)(0.45,1.0)(0.46,1.0)(0.47,1.0)(0.48,1.0)(0.49,1.0)(0.5,1.0)(0.51,1.0)(0.52,1.0)(0.53,1.0)(0.54,1.0)(0.55,1.0)(0.56,1.0)(0.57,1.0)(0.58,1.0)(0.59,1.0)(0.6,1.0)(0.61,1.0)(0.62,1.0)(0.63,1.0)(0.64,1.0)(0.65,1.0)(0.66,1.0)(0.67,1.0)(0.68,1.0)(0.69,1.0)(0.7,1.0)(0.71,1.0)(0.72,1.0)(0.73,1.0)(0.74,1.0)(0.75,1.0)(0.76,1.0)(0.77,1.0)(0.78,1.0)(0.79,1.0)(0.8,1.0)(0.81,1.0)(0.82,1.0)(0.83,1.0)(0.84,1.0)(0.85,1.0)(0.86,1.0)(0.87,1.0)(0.88,1.0)(0.89,1.0)(0.9,1.0)(0.91,1.0)(0.92,1.0)(0.93,1.0)(0.94,1.0)(0.95,1.0)(0.96,1.0)(0.97,1.0)(0.98,1.0)(0.99,1.0)(1.0,1040843.5368467863)};
\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis}[width=\onemaxplotwidthright, height=\onemaxplotheight, enlargelimits=false, grid=major, ymode=log, xlabel={\phantom{Rf, $n = 10^5$}},
             cycle list name=onemaxplotcyclenew,
             x tick label style={/pgf/number format/fixed,/pgf/number format/precision=3}]
    \addplot+ coordinates {(0.99750,1282974.728831)(0.99755,1288435.015538)(0.99760,1294008.078374)(0.99765,1299698.656375)(0.99770,1305511.793709)(0.99775,1311452.866448)(0.99780,1317527.612337)(0.99785,1323742.163988)(0.99790,1330103.085956)(0.99795,1336617.416290)(0.99800,1343292.713186)(0.99805,1350137.107548)(0.99810,1357159.362340)(0.99815,1364368.939857)(0.99820,1371776.078166)(0.99825,1379391.878305)(0.99830,1387228.404072)(0.99835,1395298.796687)(0.99840,1403617.407032)(0.99845,1412199.948830)(0.99850,1421063.676871)(0.99855,1430227.595347)(0.99860,1439712.702640)(0.99865,1449542.280477)(0.99870,1459742.237468)(0.99875,1470341.519793)(0.99880,1481372.605417)(0.99885,1492872.103094)(0.99890,1504881.484011)(0.99895,1517447.982946)(0.99900,1530625.718377)(0.99905,1544477.098655)(0.99910,1559074.606641)(0.99915,1574503.092036)(0.99920,1590862.755233)(0.99925,1608273.089163)(0.99930,1626878.173718)(0.99935,1646853.920970)(0.99940,1668418.202829)(0.99945,1691845.357088)(0.99950,1717487.560035)(0.99955,1745807.377645)(0.99960,1777429.339555)(0.99965,1813225.662354)(0.99970,1854467.454924)(0.99975,1903112.432781)(0.99980,1962410.291563)(0.99985,2038369.164344)(0.99990,2144161.348597)(0.99995,2319643.607912)(1.00000,2940300.675484)};
    \addplot+ coordinates {(0.99750,778921.38)(0.99755,783572.22)(0.99760,788317.47)(0.99765,793160.93)(0.99770,798106.66)(0.99775,803158.96)(0.99780,808322.43)(0.99785,813601.96)(0.99790,819002.77)(0.99795,824530.46)(0.99800,830191.01)(0.99805,835990.85)(0.99810,841936.89)(0.99815,848036.57)(0.99820,854297.92)(0.99825,860729.62)(0.99830,867341.07)(0.99835,874142.48)(0.99840,881144.98)(0.99845,888360.68)(0.99850,895802.87)(0.99855,903486.11)(0.99860,911426.44)(0.99865,919641.55)(0.99870,928151.08)(0.99875,936976.84)(0.99880,946143.21)(0.99885,955677.52)(0.99890,965610.59)(0.99895,975977.31)(0.99900,986817.43)(0.99905,998176.51)(0.99910,1010107.12)(0.99915,1022670.34)(0.99920,1035937.78)(0.99925,1049994.12)(0.99930,1064940.56)(0.99935,1080899.49)(0.99940,1098020.87)(0.99945,1116491.33)(0.99950,1136547.40)(0.99955,1158495.25)(0.99960,1182741.57)(0.99965,1209843.84)(0.99970,1240597.04)(0.99975,1276194.67)(0.99980,1318557.45)(0.99985,1371101.63)(0.99990,1440946.65)(0.99995,1548153.16)(1.00000,1955749.24)};
    \addplot+ coordinates {(0.9975,1.0)(0.99755,1.0)(0.9976,1.0)(0.99765,1.0)(0.9977,1.0)(0.99775,1.0)(0.9978,1.0)(0.99785,1.0)(0.9979,1.0)(0.99795,1.0)(0.998,1.0)(0.99805,1.0)(0.9981,1.0)(0.99815,1.0)(0.9982,1.0)(0.99825,1.0)(0.9983,1.0)(0.99835,1.0)(0.9984,1.0)(0.99845,1.0)(0.9985,1.0)(0.99855,1.0)(0.9986,1.0)(0.99865,1.0)(0.9987,1.0)(0.99875,1.0)(0.9988,1.0)(0.99885,1.0)(0.9989,1.0)(0.99895,1.0)(0.999,1.0)(0.99905,1.0)(0.9991,1.0)(0.99915,1.0)(0.9992,1.0)(0.99925,1.0)(0.9993,1.0)(0.99935,1.0)(0.9994,1.0)(0.99945,1.0)(0.9995,1.0)(0.99955,110.90327054914087)(0.9996,31389.990087244194)(0.99965,66742.0956123774)(0.9997,107389.03513550106)(0.99975,155201.07537987456)(0.9998,213256.53496684507)(0.99985,287175.7827012981)(0.9999,389028.02218722086)(0.99995,553792.8162295818)(1.0,1040843.5368467863)};
\end{axis}
\end{tikzpicture}
\par

